Transient Non-Use: How People in Migration Experience Digital Disconnection

People experiencing migration endure many transitions across borders, technologies, and social systems. While HCI research often emphasizes this community's adoption of technology, less attention has been paid to practices of technological non-use. This paper investigates how information and communication technologies (ICTs) are intentionally and unintentionally avoided, withheld, or not used during migration. Drawing on interviews with 32 people experiencing migration in the border city of El Paso, Texas, USA between February and May 2025, we identify a range of non-use experiences, including device, informational, and protective non-use. We extend the concept of non-use by situating it within the three phases of transitions: understanding, negotiating, and resolving. We show how ICT non-use shifts with time, risk, and institutional demands. Our analysis demonstrates that non-use functions both as a protective strategy and as a response to systemic exclusion, and concludes with design principles that anticipate non-use as both intentional and unintentional design conditions rather than as punitive failure.

==> figures/designImplicationTable.tex <==
\begin{table*}[t]
\centering
\caption{Challenging Sociotechnical Design Assumptions to Support ICT Disconnection.}
\label{tab:design_implications}
\begin{tabular}{p{3cm} p{4cm} p{4cm} p{5cm}}
\toprule
\textbf{Core assumption} & \textbf{Rationale} & \textbf{Design practice} & \textbf{Concrete example} \\
\midrule
Continuous personal device possession &
Devices are often lost, confiscated, or shared &
Do not presume continuous device possession &
Access via NGOs or shelters using PIN-based or temporary credentials without app installation \\
\midrule
Stable, continuous connectivity &
Connectivity is intermittent or unavailable &
Do not invalidate access during disconnection &
Offline-first systems that save progress and sync when connectivity returns \\
\midrule
Persistent access to identity documents &
Documents are frequently lost or withheld &
Support identity access during displacement &
Portable digital identity records accessible without physical documents \\
\midrule
Continuous presence indicates compliance &
Absence often reflects detention or forced movement &
Treat absence as predictable &
Flexible check-in windows and NGO-mediated extensions \\
\midrule
Identity is singular and centrally issued &
Centralization increases surveillance and failure risk &
Support plural, user-controlled identity &
Selective identity credentials not tied to a single authority \\
\midrule
Immediate digital verification is required &
Real-time verification assumes devices and infrastructure &
Reduce reliance on immediate verification &
Delegated or knowledge-based verification through intermediaries \\
\midrule
Eligibility expires upon disconnection &
Penalizing disconnection disproportionately harms migrants &
Preserve eligibility across absence &
Systems that retain state and allow resumption without restarting \\
\bottomrule
\end{tabular}
\end{table*}
